Ordering Chaos: Memory-Aware Scheduling of Irregularly Wired Neural Networks for Edge Devices

Recent advances demonstrate that irregularly wired neural networks from Neural Architecture Search (NAS) and Random Wiring can not only automate the design of deep neural networks but also emit models that outperform previous manual designs. These designs are especially effective while designing neural architectures under hard resource constraints (memory, MACs, . . . ) which highlights the importance of this class of designing neural networks. However, such a move creates complication in the previously streamlined pattern of execution. In fact one of the main challenges is that the order of such nodes in the neural network significantly effects the memory footprint of the intermediate activations. Current compilers do not schedule with regard to activation memory footprint that it significantly increases its peak compared to the optimum, rendering it not applicable for edge devices. To address this standing issue, we present a memory-aware compiler, dubbed SERENITY, that utilizes dynamic programming to find a sequence that finds a schedule with optimal memory footprint. Our solution also comprises of graph rewriting technique that allows further reduction beyond the optimum. As such, SERENITY achieves optimal peak memory, and the graph rewriting technique further improves this resulting in 1.68x improvement with dynamic programming-based scheduler and 1.86x with graph rewriting, against TensorFlow Lite with less than one minute overhead.

==> body/networks.tex <==
\section{Network Details}
\label{sec:networks}


% swiftnet

% randomnet

% randomnet

==> body/vwwc.tex <==
\section{Results from Visual Wake Words Challenge at CVPR 2019}
\label{sec:vwwc}
%
Figure~\ref{fig:vwwc} plots the summary of the submissions to Visual Wake Words Challenge~\cite{vwwc:2019}\footnote{Overview of the competition is provided in the link: \url{https://medium.com/tensorflow/visual-wake-words-with-tensorflow-lite-micro-8578e59ea6f9}}, and the potential gain in terms of the peak memory footprint by using our technique.
%
While the peak memory footprint was reported $200.6$KB during submission, \name improves this to $188.2$KB (both ignoring the memory allocation).

During the Visual Wake Words Challenge, the authors of the SwiftNet~\cite{swiftnet:2019}, a winner network for highest accuracy model that uses innovative compression/sparsification techniques for the next-generation embedded device, demonstrated their peak memory footprint from \emph{days of manual scheduling by a kernel-optimization expert} due to the lack of support for \emph{irregularly wired neural networks} in the current version of TensorFlow Lite.
%
This suggests that while TensorFlow Lite may be sufficient for regular topology networks, it may not be good enough for various innovations in neural architectures with irregular wirings.
%
The results suggest that using \name can \emph{automate the scheduling process with small overhead} (much faster than manual scheduling) while even \emph{exceeding the manual scheduling} in terms of the peak memory footprint. 

\begin{figure}[t!]
	\centering	
	%\vspace{-2ex} % FORMATTING
	\includegraphics[width=0.95\linewidth]{figs/vwwc_results.pdf}
	\vspace{-2ex}
	\caption{Results of the Visual Wake Words Challenge. Red arrow indicates the improvement in terms of peak memory footprint from \name, the proposed automated solution for scheduling irregularly wired neural networks.}
	\vspace{-2ex}
	\label{fig:vwwc}
\end{figure}

==> listings/naive_scheduling.tex <==
\begin{algorithm}[b!]
   \caption{Recursive Topological Ordering}
   \label{alg:naive_scheduling}
\begin{algorithmic}
   \STATE {\bfseries Input:} graph $\mathcal{G}$
   \STATE Initialize $s_0 = []$
   \STATE Initialize $S_{T0} = \{s_0\}$
   \FOR{$i=0$ {\bfseries to} $n-1$}
   \FOR{$s_i$ {\bfseries in} $S_{Ti}$}
   \STATE $z_i$ = zero-indegree($\mathcal{G}, s_i$)
   \FOR{$u_i$ {\bfseries in} $z_i$}
   \STATE $s_{i+1}$ = $s_i$.append($u_i$)
   \STATE $s_{Ti+1}$.append($s_{i+1}$)
   \ENDFOR
   \ENDFOR
   \ENDFOR
\end{algorithmic}
\end{algorithm}

